Poisson Reweighted Laplacian Uncertainty Sampling for Graph-based Active Learning

We show that uncertainty sampling is sufficient to achieve exploration versus exploitation in graph-based active learning, as long as the measure of uncertainty properly aligns with the underlying model and the model properly reflects uncertainty in unexplored regions. In particular, we use a recently developed algorithm, Poisson ReWeighted Laplace Learning (PWLL) for the classifier and we introduce an acquisition function designed to measure uncertainty in this graph-based classifier that identifies unexplored regions of the data. We introduce a diagonal perturbation in PWLL which produces exponential localization of solutions, and controls the exploration versus exploitation tradeoff in active learning. We use the well-posed continuum limit of PWLL to rigorously analyze our method, and present experimental results on a number of graph-based image classification problems.

==> RWLL Active Learning_arxiv/shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
%\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
% \usepackage[utf8]{inputenc}
% % \usepackage{geometry}
% % \geometry{a4paper, margin=1in}
% % \usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsmath, amssymb}
\usepackage{multirow}
\allowdisplaybreaks
\usepackage{xr-hyper}
\usepackage{hyperref}
\hypersetup{colorlinks,breaklinks,
             linkcolor=blue,urlcolor=blue,
             anchorcolor=blue,citecolor=blue}
\usepackage{cleveref}
\usepackage{cancel}
\usepackage{bbm}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{cite}

% % \setlength{\droptitle}{-6em}   % This is your set screw

% User defined macros
\newcommand{\mcl}{\mathcal}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\tbe}{\tilde{\mathbf{e}}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\hbu}{\hat{\mathbf{u}}}
\newcommand{\bxb}{\bar{\mathbf{x}}}
\newcommand{\byb}{\bar{\mathbf{y}}}
\newcommand{\bvb}{\bar{\mathbf{v}}}
\newcommand{\bgb}{\bar{\mathbf{g}}}
\newcommand{\mbb}{\mathbb}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lnm}{\left\|}
\newcommand{\rnm}{\right\|}
\newcommand{\hba}{\hat{\mathbf{a}}}
\newcommand{\sftau}[2]{\sqrt{\frac{\tau}{#1}}{#2}}
\newcommand{\R}{M} % interval length


\newcommand{\km}{\textcolor{blue}}
\newcommand{\jc}{\textcolor{red}}
\newcommand{\red}{\color{red}}
%\newcommand{\nc}{\normalcolor}
\newcommand{\nc}{}
 
\renewcommand{\L}{\mathcal{L}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\C}{\mathcal{D}}
\newcommand{\s}{\mathcal{S}}
\renewcommand{\epsilon}{\varepsilon}

\DeclareMathOperator*{\argmin}{arg\!min}
\DeclareMathOperator*{\argmax}{arg\!max}
\DeclareMathOperator*{\dist}{dist}
\let\div\relax
\DeclareMathOperator{\div}{div}


\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% \newsiamthm{example}{Example}
% % \newsiamthm{lemma}{Lemma}
% % \newsiamthm{proposition}{Proposition}
% % \newtheorem{proposition}[theorem]{Proposition}
\newsiamthm{policy}{Policy}
\newsiamthm{assumption}{Assumption}
%% Previously defined in our 
% \theoremstyle{definition}
% \newtheorem{remark}{Remark}
% % \newtheorem{definition}[theorem]{Definition}
% \newtheorem{problem}[theorem]{Problem}
% \newtheorem{conjecture}[theorem]{Conjecture}

% Sets running headers as well as PDF title and authors
\headers{PWLL Active Learning}{K. Miller and J. Calder}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Poisson reweighted Laplacian uncertainty sampling for graph-based active learning\thanks{Submitted to the editors DATE.
{\bf Source code: } \url{https://github.com/millerk22/rwll_active_learning}
\funding{JC was supported by NSF grant DMS:1944925,
the Alfred P. Sloan foundation, and a McKnight Presidential Fellowship}}}

% Authors: full names plus addresses.
\author{Kevin Miller\thanks{The Oden Institute of Computational Engineering and Sciences, University of Texas, Austin, TX 
  (\email{ksmiller@utexas.edu}).}
\and Jeff Calder\thanks{Department of Mathematics, University of Minnesota, Twin Cities, MN 
  (\email{jwcalder@umn.edu}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

